Pushing the Limits of Large Language Model Quantization via the Linearity Theorem

Quantizing large language models has become a standard way to reduce their memory and computational costs. Typically, existing methods focus on breaking down the problem into individual layer-wise sub-problems, and minimizing per-layer error, measured via various metrics. Yet, this approach currently lacks theoretical justification and the metrics employed may be sub-optimal. In this paper, we present a "linearity theorem" establishing a direct relationship between the layer-wise $\ell_2$ reconstruction error and the model perplexity increase due to quantization. This insight enables two novel applications: (1) a simple data-free LLM quantization method using Hadamard rotations and MSE-optimal grids, dubbed HIGGS, which outperforms all prior data-free approaches such as the extremely popular NF4 quantized format, and (2) an optimal solution to the problem of finding non-uniform per-layer quantization levels which match a given compression constraint in the medium-bitwidth regime, obtained by reduction to dynamic programming. On the practical side, we demonstrate improved accuracy-compression trade-offs on Llama-3.1 and 3.2-family models, as well as on Qwen-family models. Further, we show that our method can be efficiently supported in terms of GPU kernels at various batch sizes, advancing both data-free and non-uniform quantization for LLMs.

==> srcs/data/dynamic_algorithm.tex <==
\begin{algorithm}
\caption{Optimal Dynamic Bitwidth}\label{alg:cap}
\hspace*{\algorithmicindent} \textbf{Input:} set of model subdivisions $\{S_i\}$, metric $\mathcal{M}$, bitwidths and expexted L2 errors $\{(B_g,L_g)|g \in \mathcal{G}\}$ for a set of grids $\mathcal{G}$, total bitwidth budged $\mathcal{B}$.

\hspace*{\algorithmicindent} \textbf{Output:} mapping from subdivision to grids $\{S_i \longrightarrow \mathcal{G}\}$

\begin{algorithmic}
\For{$S_i \in \{S_i\}$}
    \State Measure $\mathcal{M}(S_i + \varepsilon_i)$ for a range of noise scales $\varepsilon_i$.
    \State Calculate the slope $\sigma_i$ of the linear fit of $\mathcal{M}$ as a function of $\varepsilon_i$.
\EndFor

\State ...
\State Profit!

\end{algorithmic}
\end{algorithm}


==> srcs/data/grids_comparison.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of entropy-optimal (NF4), L1-optimal (AF4) and MSE-optimal (EDEN, HIGGS) grids on Llama-3.1-8B quantization with Hadamard incoherence pre-processing.}
\vspace{0.3cm}
\label{tab:grids_comparison}
\begin{tabular}{|l|cccc|}
\hline
\multicolumn{1}{|l|}{Grid} & L2 error & L1 error & Entropy & \multicolumn{1}{l|}{WK2 PPL} \\ \hline
NF4                        & 0.156    & 0.110    & 4.00    & 7.42                         \\ \hline
AF4                        & 0.108    & 0.094    & 3.91    & 6.27                         \\ \hline
EDEN                       & 0.098    & 0.099    & 3.76    & 6.13                         \\ \hline
HIGGS (2D)                 & 0.088    & 0.088    & 3.90    & 6.04                         \\ \hline
\end{tabular}

\end{table}


==> srcs/data/methods_comparison.tex <==
\begin{table*}
\centering
\caption{Comparison of NF4, AF4, EDEN and HIGGS Meta-Llama-3.1-8B quantization.}
\vspace{0.3cm}
\label{tab:methods_comparison}
\begin{tabular}{l|ccccccc}
\hline
\multicolumn{1}{|l|}{Method} & \multicolumn{1}{l}{Bitwidth} & \multicolumn{1}{l}{WK2 PPL$\downarrow$} & \multicolumn{1}{l}{WG$\uparrow$} & \multicolumn{1}{l}{PiQA$\uparrow$} & \multicolumn{1}{l}{ArcE$\uparrow$} & \multicolumn{1}{l}{ArcC$\uparrow$} & \multicolumn{1}{l|}{MMLU$\uparrow$} \\ \hline
HQQ (gs64)                   & 3.25                         & 7.317                                   &                                  &                                    &                                    &                                    & 56.41                               \\
EDEN (1d9)                   & 3.19                         & 7.501                                   & 69.93                            & 76.99                              & 77.19                              & 44.97                              & 52.51                               \\
HIGGS (2d88)                 & 3.25                         & 7.110                                   & 73.01                            & 77.04                              & 76.35                              & 44.11                              & 57.61                               \\
HIGGS (3d830)                & 3.25                         & 6.807                                   &                                  &                                    &                                    &                                    & 60.06                               \\ \hline
AF4 (gs1024)                 & 4.00                         & 6.194                                   &                                  &                                    &                                    &                                    & 61.51                               \\
HQQ (gs1024)                 & 4.00                         &                                         &                                  &                                    &                                    &                                    & 57.78                               \\
EDEN (1d16)                  & 4.00                         & 6.142                                   &                                  &                                    &                                    &                                    & 61.62                               \\
HIGGS (2d256)                & 4.00                         & 6.016                                   &                                  &                                    &                                    &                                    & 63.11                               \\ \hline
NF4 (gs64)                   & 4.25                         & 5.967                                   & 73.00                            & 79.49                              & 81.57                              & 51.79                              & 63.30                               \\
AF4 (gs64)                   & 4.25                         & 5.953                                   & 74.43                            & 79.27                              & 80.85                              & 49.74                              & 63.19                               \\
HQQ (gs64)                   & 4.25                         & 6.001                                   & 73.95                            & 79.82                              & 81.44                              & 50.00                              & 63.78                               \\
EDEN (1d19)                  & 4.25                         & 5.978                                   & 73.32                            & 79.60                              & 81.02                              & 50.26                              & 63.52                               \\
HIGGS (2d361)                & 4.25                         & 5.908                                   & 74.27                            & 79.43                              & 81.48                              & 50.51                              & 63.63                               \\ \hline
Int8                         & 8.00                         & 5.612                                   & 73.48                            & 80.14                              & 81.23                              & 51.11                              & 65.31                               \\
HQQ (gs64)                   & 8.25                         & 5.609                                   & 73.56                            & 80.09                              & 81.11                              & 51.11                              & 65.40                               \\
EDEN (1d256)                 & 8.00                         & 5.608                                   & 73.64                            & 79.98                              & 81.57                              & 51.28                              & 65.35                               \\ \hline
FP16                         & 16.00                        & 5.607                                   & 73.72                            & 79.98                              & 81.44                              & 51.19                              & 65.36                              
\end{tabular}
\end{table*}

